Brave: Byzantine-Resilient and Privacy-Preserving Peer-to-Peer Federated Learning

Federated learning (FL) enables multiple participants to train a global machine learning model without sharing their private training data. Peer-to-peer (P2P) FL advances existing centralized FL paradigms by eliminating the server that aggregates local models from participants and then updates the global model. However, P2P FL is vulnerable to (i) honest-but-curious participants whose objective is to infer private training data of other participants, and (ii) Byzantine participants who can transmit arbitrarily manipulated local models to corrupt the learning process. P2P FL schemes that simultaneously guarantee Byzantine resilience and preserve privacy have been less studied. In this paper, we develop Brave, a protocol that ensures Byzantine Resilience And privacy-preserving property for P2P FL in the presence of both types of adversaries. We show that Brave preserves privacy by establishing that any honest-but-curious adversary cannot infer other participants' private data by observing their models. We further prove that Brave is Byzantine-resilient, which guarantees that all benign participants converge to an identical model that deviates from a global model trained without Byzantine adversaries by a bounded distance. We evaluate Brave against three state-of-the-art adversaries on a P2P FL for image classification tasks on benchmark datasets CIFAR10 and MNIST. Our results show that the global model learned with Brave in the presence of adversaries achieves comparable classification accuracy to a global model trained in the absence of any adversary.

==> sections/Preliminaries.tex <==
\section{Security Perlimiaries}
 In this section, we give the security preliminaries for solving the proposed secure and private weight aggregation problem. First, we define trim-secure, which ensures the robustness of the model aggregation, i.e., the global model is $\epsilon$-convergence. Then, we introduce distributed consensus that ensures agreement in the context of the distributed system.
 
\subsection{Trim-Secure Weight} 

\textcolor{red}{Add some proof(provable security guarantees) here.}

\subsection{Distributed Consensus and Log Replication}
The Trim-secure weight can provide security guarantees as we have proved. Now we focus on achieving agreement in distributed systems. 

The pursuit of consistency reminds us of the classic distributed consensus problem first proposed in \cite{pease_reaching_1980}, which investigates how to guarantee the nodes agree on an identical value, despite the existence of faulty nodes and unreliable communication links. Theoretically, distributed consensus with Byzantine fault tolerance can be solved under $t < N/3$ without authentication under synchronous network assumption \cite{lamport2019byzantine}.
In particular, the \textit{log replication} problem studies how to let the log entries from clients be identically replicated to all nodes with \textit{safety} and \textit{liveness} guarantee, where safety means log entries replicated to all nodes are the same, and liveness means the process will continue without getting stuck. Therefore, we can regard the values (and other related messages) to be broadcast as logs, and replicate them to all participants via an existing log replication protocol to ensure consistency (i.e., safety).

As an enduring theme in the field of distributed systems, distributed consensus has also received wider attention in recent years due to the development of blockchain technology, and many practical log replication consensus algorithms have emerged. Today, using consensus for reliable broadcasting is no longer expensive: since PBFT \cite{castro1999practical}, numerous byzantine-fault-tolerance (BFT) log replication protocols (e.g., Prime \cite{amir2010prime}, Zyzzyva \cite{kotla2007zyzzyva}, and SBFT \cite{gueta2019sbft}) have been proposed to reduce communication overhead, and Hotstuff \cite{yin2019hotstuff} even achieves a linear communication complexity as the state of the art.

As the main concern of our work is to design a secure gradient aggregation mechanism, we do not focus on designing a consensus protocol for reliable broadcast. Instead, any existing BFT log replication protocols can be implemented in our solution to reliably broadcast the values to all participants with consistency, and we call this process \textit{Byzantine Broadcast}. Since the log replication generally guarantees safety and liveness properties (if not, a view-change protocol would probably be executed), we may assume it is reliable. For a concise presentation of our solution, we abstract Byzantine broadcast as a reliable broadcast layer already existing in the participants, and keep it independent of our solution.


==> sections/challenge.tex <==
\subsection{Challenges}
\label{subsec: challenges}

Solving Problem \ref{problem:formulation} is non-trivial due to the following challenges.
First, the existing Byzantine resilient FL frameworks \cite{blanchard2017machine,yin2018byzantine} are not readily applicable to peer-to-peer FL.
The aforementioned approaches rely on a centralized server to collect information from all participants and then eliminate the outliers to update the global model.
However, such a centralized server does not exist in peer-to-peer FL considered in this paper, leading to partial information on local models perceived by each benign participant.
Second, a Byzantine adversary can intelligently manipulate its local model when communicating with different participants such that the information collected by the benign participants becomes compromised to different extents. 
Furthermore, although letting the participants truthfully reveal their local models may benefit identifying and isolating Byzantine adversaries, this allows the passive adversaries to infer the private training data owned by the other participants.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% We have a few challenges in designing a protocol that satisfies information-theoretic privacy and resilience with the existence of adversaries. 

% First, it goes without saying that in classic federated learning without privacy concerns, achieving $\epsilon$-convergence is quite easy: the central server just needs to remove the outliers according to the statistical properties of the input models of the participants. There are some prior works already proposed various solutions and proved their robustness to Byzantine adversaries. For example, \textit{Krum} \cite{blanchard2017machine} selects the gradient that minimizes the sum of squared distances to its $n-f$ closest gradients. On the other hand, \textit{Trimmed Mean} \cite{yin2018byzantine} is a coordinate-wise aggregation rule that considers each model parameter individually. Within each parameter, it removes the largest $f$ and the smallest $f$ values, and then computes the mean of the remaining $n-2f$ values as the value of the corresponding parameter in the global model. Another similar coordinate-wise aggregation idea is \textit{median}. It sorts the values of each individual parameter in all local model updates and considers the median value to be the parameter to be the global model. Such solutions give us the intuition to perform sorting of all inputs. Here, we meet the first challenge: in peer-to-peer FL, how can we sort all models correctly while achieving information-theoretic secrecy, i.e., not disclosing its true local model?

% In addition, sorting is inadequate for aggregating a global model. As indicated in Equation \eqref{equation directly average weight}, the global model update of one participant requires a local model from other participants. Recall that Byzantine adversaries may send manipulated or even different local models to other participants, it is challenging to perform a privacy-preserving sum with Byzantine-fault tolerance. Therefore, the second challenge arises, that is how to calculate the mean of the input models without a central aggregator, and how to ensure the calculated global model among different nodes is the same (i.e., agreement)? 

% The most challenging problem occurs in the middle of the two problems above: a clever adversary could input a normal value to participate in the sorting, and then input an outlier to bias with the final aggregated model when averaging, which made the previous sorting useless. However, since the inputs are private, there is no way to find and blame the adversary. So the third problem is: even if we get a correct ranking, how can we guarantee that the participants input the same model in sorting and averaging? 


==> sections/overview.tex <==
\subsection{Protocol Overview}
% The pursuit of consistency reminds us of the classic distributed consensus problem first proposed in \cite{pease_reaching_1980}, which investigates how to guarantee the nodes agree on an identical value, despite the existence of faulty nodes and unreliable communication links. 
% In particular, the \textit{log replication} problem studies how to let the log entries from clients be identically replicated to all nodes with \textit{safety} and \textit{liveness} guarantee, where safety means log entries replicated to all nodes are the same, and liveness means the process will continue without getting stuck. Therefore, we can regard the values (and other related messages) to be broadcast as logs, and replicate them to all participants via an existing log replication protocol to ensure consistency (i.e., safety).

% As an enduring theme in the field of distributed systems, the distributed consensus has also received wider attention in recent years due to the development of blockchain technology, and many practical log replication consensus algorithms have emerged. Today, using consensus for reliable broadcasting is no longer expensive: since PBFT \cite{castro1999practical}, numerous byzantine-fault-tolerance (BFT) log replication protocols (e.g., Prime \cite{amir2010prime}, Zyzzyva \cite{kotla2007zyzzyva}, and SBFT \cite{gueta2019sbft}) have been proposed to reduce communication overhead, and Hotstuff \cite{yin2019hotstuff} even achieves a linear communication complexity as the state of the art.

% As the main concern of our work is to design a secure gradient aggregation mechanism, we do not focus on designing a consensus protocol for reliable broadcast. Instead, any existing BFT log replication protocols can be implemented in our solution to reliably broadcast the values to all participants with consistency, and we call this process \textit{Byzantine Broadcast}. Since the log replication generally guarantees safety and liveness properties (if not, a view-change protocol would probably be executed), we may assume it is reliable. For a concise presentation of our solution, we abstract Byzantine broadcast as a reliable broadcast layer already existing in the participants, and keep it independent of our solution.

The overall structure of \texttt{Brave} is illustrated in Fig. \ref{fig: algorithm flow}.
All stages of \texttt{Brave} require the participants to broadcast messages via a module named BFT broadcast (the grey color box in Fig. \ref{fig: algorithm flow}).
BFT broadcast utilizes Byzantine-fault-tolerant (BFT) distributed consensus algorithms, which follow a propose-vote paradigm \cite{shi2020foundations}.
In the BFT broadcast, the message sent by each participant is treated as a proposal.
All participants will incorporate the proposal to their local information set as long as more than $N-f$ participants agree with the proposal.
Typical implementations of the BFT distributed consensus algorithms include PBFT \cite{castro1999practical}, Zyzzyva \cite{kotla2007zyzzyva}, and Hotstuff \cite{yin2019hotstuff}.
Using the state-of-the-art implementation of BFT broadcast, Hotstuff \cite{yin2019hotstuff}, \texttt{Brave} guarantees that all participants will reach an agreement on messages sent by the participants, with communication complexity linear in $N$.

\begin{figure}[htbp]
  \centering 
  \includegraphics[width=0.5\textwidth]{algorithm flow.pdf}
  \caption{This figure shows the overall workflow of \texttt{Brave}. Our proposed protocol, \texttt{Brave}, consists of three stages. All participants are required make commitments on their claimed local models (Stage \raisebox{.5pt}{\textcircled{\raisebox{-.9pt} {1}}} in Fig. \ref{fig: algorithm flow}). The privacy-preserving trimming stage (Stage \raisebox{.5pt}{\textcircled{\raisebox{-.9pt} {2}}}) sorts the claimed local models and trims the largest and lowest $f$ entries without disclosing their true values. The final Stage  \raisebox{.5pt}{\textcircled{\raisebox{-.9pt} {3}}}, agreement and verification, validates the local models that are not trimmed in Stage 2, and updates the global model.}
  \label{fig: algorithm flow} 
\end{figure}



\begin{figure*}[b]
  \centering 
  \includegraphics[width=1\textwidth]{communication structure.pdf}
  \caption{This figure depicts a P2P FL with six participants $\{P_0,\ldots,P_5\}$ and illustrates 
   the schematic message flow of \texttt{Brave}. In this example, $P_5$ is a Byzantine adversary. In Stage 1, all participants broadcast their commitments of local models to BFT broadcast module. In Stage 2, the participants first exchange messages among themselves using the point-to-point communication network. After that, they send a set of relationships among local models to BFT broadcast. In Stage 3, all participants receive messages from BFT broadcast to aggregate the local models and update the global model.
   In Stage 2 of \texttt{Brave}, the local model of $P_5$ is trimmed by our protocol, leading to limited bias to P2P FL.}
  \label{fig: communication structure} 
\end{figure*}

\begin{lemma}
If $N>3f+2$, then the messages sent by a participant via BFT broadcast will be received identically by benign participants.
\label{lemma BFT agreement}
\end{lemma}
\begin{proof}
According to \cite{lamport2019byzantine}, consensus can be reached if $N > 3f$ without authentication under synchronous network assumption, and identical information can be received. Thus the lemma follows given $N>3f+2>3f$.
\end{proof}


\texttt{Brave} consists of three stages that occur sequentially: \textit{commitment}, \textit{privacy-preserving trimming}, and \textit{aggregation and verification}.
We describe these stages below.
\begin{enumerate}
    \item \textit{Commitment:} Each $P_i$ updates its local model ${w}_i$, and then generates a commitment of ${w}_i$ using the Pedersen commitment scheme \cite{feigenbaum_non-interactive_1992}. It then sends the commitment via the BFT broadcast module as shown in Fig. \ref{fig: algorithm flow}. Thereafter $P_i$ is not allowed to edit its commitment. In the meantime, $P_i$ receives the commitments from all $P_j$ where $j\neq i$.
    \item \textit{Privacy-Preserving Trimming:} Each $P_i$ generates a `masked' message for every $P_j\in\mathbb{P}\setminus\{P_i\}$, and then forwards to all other participants. 
    Using the masked messages, \texttt{Brave} sorts all participants' local models coordinate-wise.
    Then the protocol trims the largest and smallest $f$ local models along each dimension, and uses the remaining ones for the next stage.
    % \item \textit{Privacy-preserving trimming:} Each $P_i$ generates a `masked' message for every $P_j\in\mathbb{P}\setminus\{P_i\}$, and then forwards to all other participants. After receiving the masked messages from other participants, each participant verifies the message and performs a secure pairwise comparison scheme to coordinate-wisely compare the local models of $P_p$ and $P_q$ for all $p$ and $q$ without disclosing the true values of local models owned by $P_p$ and $P_q$. The comparison results maintained by each participant are then sent to the BFT broadcast for agreement. Each participant next trims the sorted local models coordinate-wise by removing the $f$ largest and smallest entries of the masked local models.
    \item \textit{Aggregation and Verification:} $P_i$ generates a private one-time pad \cite{bonawitz2017practical} and masks the non-trimmed dimensions of its local model before sending them to BFT broadcast. 
    After receiving the masked dimensions from other participants, each $P_i$ adds the masked values coordinate-wise and verifies authenticity. 
    Finally, each $P_i$ computes the global model if the summations of the masked values are authenticated.
\end{enumerate}

Fig. \ref{fig: communication structure} illustrates the schematic message flow of \texttt{Brave} when applied to a P2P FL with six participants.






% Once a participant sends a message to BFT broadcast, the other replicas will incorporate the message to their local information set as long as more than $N-f$ participants agree.
% Furthermore, the BFT broadcast module will guarantee the participants to reach an agreement on the global model after the P2P FL converges with communication complexity linear in $N$.


% In this stage, each $P_i$ generates $N-1$ secondary commitment messages, with each corresponding to a participant in $\mathbb{P}\setminus \{P_i\}$.
% The participant next `masks' its local model ${w}_i(t)$ using a secondary commitment message, and sends the masked local model to all other participants.






% In the first commitment stage, each participant implements a cryptography primitive called \textit{commitment scheme} to ``lock'' the local model to prevent an adversary participant from modifying it in later stages. Then in the next \textit{privacy-preserving trimming stage}, participants performs a secure multi-party sorting to coordinate-wise rank the local model of all participants and choose the participants sorted in the middle region as ``contributors''. In the last \textit{summation} stage, participants who are contributors sum their local model by sending values masked by the one-time pad, and then all nodes verify the authenticity of the aggregated global model by opening the commitments that they sent at the first stage.
% We will describe the procedure in detail in the following part of this section.

% 之前expensive，写complexity是多少

% 所有都会用这个broadcast
% consensus
% linear的
% reach 了 consensus，所以我们用它保证agreement
% 不要停留在历史的尘埃中，we do we do we do we do we do
% 我们的是好的，证明了这个complexity

% Our proposed protocol implement the distributed consensus algorithm as a way of reliably broadcasting the messages, which realizes the agreement property defined in Section \ref{sec: problem formulation}. A distributed consensus algorithm guarantees all participants agree on an identical value (or a message), despite the existence of faulty (i.e., crash or Byzantine) participants. 
% Generally, most distributed consensus algorithms works in a propose-vote paradigm \cite{shi2020foundations}, where a leader propose the value or message needed to be agreed on, and all other participants vote for it. When the leader is faulty, the view change will occur to rotate the leader.
% In the past, it was considered expensive to achieve a reliable broadcast via distributed consensus, because the communication complexity was more than $O(N^2)$. However, the recently proposed Hotstuff \cite{yin2019hotstuff} achieves a linear communication complexity, so using consensus for reliable broadcasting in a distributed system is no longer expensive. Note that theoretically, distributed consensus with Byzantine fault tolerance (BFT) can be solved under $t < N/3$ without authentication under synchronous network assumption \cite{lamport2019byzantine}, so we can guarantee the consistency of the message broadcasting under the Inequality \ref{equation N>3f+2}.


% 具体共识是怎么实现的

% protocol是什么，每个agent都要follow 有几个模块
% Stage 1实现什么 mask information 接下来哪个section会讲，commitment
% 收到info 之后 Stage 2 Sort MPC
% high level
% Byzantine 广播
% 我们adopt了perdersen commitment，定义 technic是怎么工作的，不要review background
% 每个当作一个模块


% The procedure of our protocol is demonstrated in Figure \ref{fig: algorithm flow}. The protocol has three stages: commitment, comparison \& sorting, and summation \& verification.
% We assume the dataset is i.i.d., and the initial model and step size $\eta$ have been consistently distributed before the training starts. In each iteration, the participants first update the local model using the current global model and its own dataset, then commit the gradient via BFT log replication. 
% After the commitment, we divide the procedure into two sub-processes: i) comparison \& sorting and ii) summation \& result verification, where the committed message served as a constraint throughout the process to ensure consistent input. In the end, every participant performs a gradient descent update on the model parameter with the aggregated trim-secure gradient. 

% \begin{figure}[htbp]
%   \centering 
%   \includegraphics[width=0.3\textwidth]{algorithm flow.pdf}
%   \caption{The structure of our approach.}
%   \label{fig: algorithm flow} 
% \end{figure}

% We assume the dataset is i.i.d., and the initial model and step size $\eta$ have been consistently distributed before the training starts.
% Note that we use the function $\texttt{BFT-Broadcast}(m)$ in our protocol to represent the process of implementing the BFT log replication protocol to reliably broadcast message $m$. We colored the Byzantine broadcast in blue in the pseudo-code for cross-referencing to Figure \ref{fig: communication structure}.

%  given:
% \begin{equation}
% 	N>3f+2,
% 	\label{equation N>3f+2}
% \end{equation}
% where $N$ is the total number of participants and $f$ is the maximum number of adversaries. Figure \ref{fig: communication structure} shows our protocol when applied to one iteration of P2P FL involving six participants with one ($P_5$) being faulty.
% % , which consists of six participants, and $P_5$ in red is a faulty participant.  


==> sections/security.tex <==
\section{Byzantine Resilience Analysis}
\label{sec: Byzantine Resilience Analysis}

% First, we consider the input weight ${w}_i \in \mathbb{R}$, i.e., ${w}_i$ is a one-dimensional vector, and assume w.l.o.g. that system inputs are different, so we can rank input weights from different participants.
% \begin{definition}[Trim-Secure Value]
%     Given the system inputs $w_1,w_2, \dots, w_N \in \mathbb{R}$, where $w_1<w_2<\dots <w_N$. We say $w_i$ is a trim-secure value if $w_{f}<w_i<w_{N-f}$, where $f$ is the maximum fault tolerance.
% \end{definition}

% Intuitively, a value is trim-secure if it is neither the smallest $f$ nor the largest $f$ among all inputs. The main idea is that when the dataset is independent and identically distributed (i.i.d.), the weight updates from non-faulty participants tend to be close to the true weight, while updates from adversaries could be arbitrary. Therefore, extreme values possibly introduced by at most $f$ malicious nodes can be eliminated by sorting all inputs and only taking the middle $N-2f$ values. 

% Note that generally, the model parameter ${w}_i$ is a vector. Therefore, we consider a more general case when the weight ${w}_i \in \mathbb{R}^m$, i.e., ${w}_i$ is an m-dimensional vector, and give the definition of the trim-secure weight.

\begin{definition}[Trim-Secure Weight]
Given the system inputs ${w}_1,{w}_2, \dots, {w}_N \in \mathbb{R}^m$, we say ${w}_i$ is a trim-secure weight if $\forall k \in \{1,2,\dots,m\}$, the $k$-th coordinate ${w}_{ik}$ of ${w}_i$ is a trim-secure value within that coordinate.
\end{definition}

\begin{lemma}[Local Non-Forgeability]
	If a non-faulty participant $P_i$ broadcasts $w^k_p>w^k_q$ at dimension $k$, then the claimed local model of $P_p$ w.r.t. to $\mathcal{W}_p$ is greater than that of $P_q$ at dimension $k$.
	\label{property non-forgeability}
\end{lemma}
\begin{proof}
Consider three cases when i) both $P_p$ and $P_q$ are benign, ii) either $P_p$ or $P_q$ is Byzantine, iii) both $P_p$ and $P_q$ are Byzantine, and they may collude.
We show proof of case iii), and similar approaches can be applied to cases i) and ii).

Assume in dimension $k$, $w^k_{p}>w^k_{q}$. To pass the authentication of a non-faulty $P_i$, $P_p$ and $P_q$ must find \textit{a)} another valid pairs $w_{q}'$ or $w_{p}'$ such that $w^{k'}_{q}>w^{k'}_{p}$ but $w^k_{q}<w^k_{p}$, or
\textit{b)} another valid vector $v_{qp}'+v_{pq}'$ such that $v^{k'}_{qp}+v^{k'}_{pq}-v^k_{qp}-v^k_{pq}>w^k_{p}-w^k_{q}$.
However, Lemma \ref{lemma Pedersen commitment} indicates that the Pedersen commitment scheme is computational binding, i.e., a Byzantine participant can not find another value that opens the same commitment.
Therefore, both \textit{a)} and \textit{b)} are impossible, and the comparison result of $d_{pq}$ and $d_{qp}$ truly reflects the relationship between the claimed local model $w_p$ and $w_q$.
\end{proof}

Next, we move from a local perspective to a holistic one considering $N>3t+2$. We first prove the adversary cannot forge a comparison, as shown in the following proposition. 

\begin{proposition}[Global Non-Forgeability]
\label{property Global Non-Forgeability}
	If $w^k_p>w^k_q$ is accepted by a non-faulty participant $P_i$ in Line \ref{codeline accept wp>wq} of Algorithm \ref{Participant Only: algorithm aggregator comparison and sorting}, then the claimed local model of $P_p$ w.r.t. to $\mathcal{W}_p$ is greater than that of $P_q$ at dimension $k$ given $N<3f+2$.
\end{proposition}
\begin{proof}
If $P_p$ and $P_q$ are both non-faulty, the above argument trivially holds. Then we prove by contradiction to show that the Byzantine adversary cannot forge the result. Assume $w^k_p > w^k_q$ is true, and a non-faulty participant receives a wrong relationship $w^k_p < w^k_q$ for more than $f$ times. Recall that there are at most $f$ faulty participants, so there is at least one non-faulty participant that also broadcast $w^k_p < w^k_q$, which contradicts Lemma \ref{property Global Non-Forgeability}.
\end{proof}

We then present a property that affirms the relationship within the non-faulty participants, and thus guarantees the liveness. In other words, even if the faulty participants do not involve (e.g., remain silent), a benign participant $P_i$ can construct a sequence $\mathcal{S}_i$ regardless of the behaviors of Byzantine adversaries. 

\begin{proposition}[Liveness]
\label{property non-faulty closedness}
If $P_p$ and $P_q$ are non-faulty participants and assume w.l.o.g. $w^k_p>w^k_q$, then $w^k_p>w^k_q$ will be accepted by all non-faulty participants in Line \ref{codeline accept wp>wq} of Algorithm \ref{Participant Only: algorithm aggregator comparison and sorting} given $N>3t+2$.
\end{proposition}
\begin{proof}
Since $P_p$ and $P_q$ are non-faulty, they will follow the protocol and send $m_{pq}$ and $m_{pq}$ that can be authenticated to other participants. As $N>3t+2$, apart from $P_p$ and $P_q$, there are at least $(N-2)-f>2f$ non-faulty nodes that will respond with $w^k_p>w^k_q$. Therefore, all non-faulty participants would receive more than $2f$ times $w^k_p>w^k_q$ and accept $w^k_p>w^k_q$.
\end{proof}

Now we come to the agreement proposition.

\begin{proposition}[Agreement on Pairwise Relationships]
	The accepted relationships of all non-faulty participants are identical given $N>3f+2$.
	\label{property Agreement on Pairwise Comparison Result}
\end{proposition}
\begin{proof}
	This property is guaranteed by the BFT broadcast given $N>3f$, as shown in Lemma \ref{lemma BFT agreement}.
\end{proof}

With Proposition \ref{property Global Non-Forgeability} and Proposition \ref{property Agreement on Pairwise Comparison Result}, we can now conclude that the relationships among non-faulty participants are \textit{correct} and \textit{identical}. Therefore, a ranking can be performed, where the inputs from non-faulty participants are guaranteed to be included as shown in Property \ref{property non-faulty closedness}. Furthermore, we have the following corollary of Property \ref{property Agreement on Pairwise Comparison Result}.

\begin{corollary}[Agreement on Sorting]\label{property agreement on ranking}
	Given any non-faulty participants $P_i$ and $P_j$, if $N>3f+2$ holds, then Brave guarantees the sorting results $\mathcal{S}^k_i=\mathcal{S}^k_j$ for all $k$, i.e., the sorting of all non-faulty participants is identical.
\end{corollary}

\begin{proposition}[Agreement on Global Model]
The global model $w$ of all non-faulty participants is identical given $N>3f+2$.
\label{property agreement on global model}    
\end{proposition}
\begin{proof}
    Given Corollary \ref{property agreement on ranking} and Lemma \ref{lemma BFT agreement}, $\mathcal{S}_i^k=\mathcal{S}_j^k$, $\bar{w}_i^k=\bar{w}_j^k$ and $\bar{r}_i^k=\bar{r}_j^k$ for all non-faulty participants $P_i$ and $P_j$. Thus $\bar{w}^k$ calculated in Line \ref{line 12 algorithm 3} is identical among non-faulty participants, who would later obtain the same verification result in \ref{line 14 algorithm 3}. Therefore, the global model $w$ is also identical.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In what follows, we prove Byzantine resilience of Brave.
Using Proposition \ref{property agreement on ranking} and \ref{property agreement on global model}, we have that own identical $\mathcal{S}_i^k=\mathcal{S}_j^k$ for all non-faulty participants $i,j$. 
They further hold identical global model $w(t)$ for all iteration $t$. 
Consider an arbitrary non-faulty participant. 
If $w(t)$ is $z$-sub-exponential, then using \cite[Lemma 3]{yin2018byzantine} yields 
\begin{equation*}
    |w^k - w^{k^*}|\leq \frac{t+3f \delta/N}{1-2f/N}
\end{equation*}
holds for each dimension $k$ with probability at least $1-2\exp\{-(N-f)\min_{i}|\mathcal{D}_i|\min\{\frac{t}{2z},\frac{t^2}{2z^2}\}\}-2(N-f)\exp\{\min_i|\mathcal{D}_i|\min\{\frac{\delta}{2z},\frac{\delta^2}{2z^2}\}\}$.
By using the definitions of $\|\cdot\|$ and union bound, we have that
\begin{equation*}
    \|w^k - w^{k^*}\|\leq \sqrt{m}\frac{t+3f \delta/N}{1-2f/N}
\end{equation*}
holds with probability at least $1-2m\exp\{-(N-f)\min_{i}|\mathcal{D}_i|\min\{\frac{t}{2z},\frac{t^2}{2z^2}\}\}-2(N-f)m\exp\{\min_i|\mathcal{D}_i|\min\{\frac{\delta}{2z},\frac{\delta^2}{2z^2}\}\}$ for any $t,\delta\geq 0$.


% \begin{theorem}
% The committed input $w$ of any contributor is a \textit{trim-secure value}.
% \label{theorem contributor trim secure}
% \end{theorem}
% \begin{proof}
%     We denote the input of the node that ranked $t+1$-th is $\overset{*}{w}_{t+1}$, and that ranked $N^{'}-t$-th is $\overset{*}{w}_{N'-t}$. Since $N^{'} \leq N$, it is possible that there are some nodes missing in the final ranking, but their actual values $w$ are within $w \leq w_{t+1}$. So $\overset{*}{w}_{t+1} \geq w_{t+1}$. Similarly, $\overset{*}{w}_{N'-t} \leq w_{N-t}$. Since the minimum and maximum contributors are bounded by the definition of trim-secure values, the input gradient of any contributor is a trim-secure value.
% \end{proof}
